Sliced-Wasserstein Estimation with Spherical Harmonics as Control Variates

The Sliced-Wasserstein (SW) distance between probability measures is defined as the average of the Wasserstein distances resulting for the associated one-dimensional projections. As a consequence, the SW distance can be written as an integral with respect to the uniform measure on the sphere and the Monte Carlo framework can be employed for calculating the SW distance. Spherical harmonics are polynomials on the sphere that form an orthonormal basis of the set of square-integrable functions on the sphere. Putting these two facts together, a new Monte Carlo method, hereby referred to as Spherical Harmonics Control Variates (SHCV), is proposed for approximating the SW distance using spherical harmonics as control variates. The resulting approach is shown to have good theoretical properties, e.g., a no-error property for Gaussian measures under a certain form of linear dependency between the variables. Moreover, an improved rate of convergence, compared to Monte Carlo, is established for general measures. The convergence analysis relies on the Lipschitz property associated to the SW integrand. Several numerical experiments demonstrate the superior performance of SHCV against state-of-the-art methods for SW distance computation.

==> conventions.tex <==

%%% Checklist for consistency
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Monte Carlo in place of MC
% i.e. NOT italics
% Section 6: keep and upgrade Propositions
% Remove Proposition on mean invariance, phrase it as a sentence.


% dP(s) vs P(ds) (DONE)
% Algorithms vs text (DONE) 
% (\theta^star)_\sharp vs \theta^star_\sharp (DONE)

%%%%%%%%%%%% To-Do list %%%%%%%%%%%% 
% Write abstract
% Polish "Contributions" in the introduction
% Add comments after Theorems/Corollary in Section 6
% Write Conclusion with open research questions such as
% - SW with other than uniform distributions (use importance sampling weights
% - Gradient estimation 

==> progress_work.tex <==
\section{Work in Progress}



Consider particles $\theta_1,\ldots,\theta_n \in \sphere$ and denote $f_n = (f_{\mu,\nu}^{(p)}(\theta_1),\ldots,f_{\mu,\nu}^{(p)}(\theta_n))$. Let $\Pi_n = \Phi(\Phi^\top \Phi)^{-1} \Phi^\top$ be the $n \times n$ projection matrix on the column space of the matrix $\Phi=(\varphi_j(\theta_i))$. The SHCV estimate can be rewritten as
$$ \mathrm{SHCV}_n(\mu,\nu) = \argmin_{\alpha \in \rset} \|(I_n - \Pi_n)(f_n-\alpha \1_n)\|_2^2
$$
and is uniquely defined as soon as $\1_n$ is not an element of the column space of $\Phi$. In this case, we have $$
\mathrm{SHCV}_n(\mu,\nu) = \frac{\1_n^\top (\Int-\Pi)f_n}{\1_n^\top (\Int-\Pi)\1_n} $$
\begin{proposition}(Quadrature rule) The $\mathrm{SHCV}$ estimate of $\slice_p^p(\mu,\nu)$ based on particles $\theta_1,\ldots,\theta_n \sim \mathcal{U}(\sphere)$ is a linear integration rule $\mathrm{SHCV}_n(\mu,\nu) = \sum_{i=1}^n w_{n,i} f_{\mu,\nu}^{(p)}(\theta_i)$ where the weights $(w_{n,i})_{i=1}^n$ do not depend on the integrand $f^{(p)}_{\mu,\nu}$ and are given by $w_n =[(\Int-\Pi)\1_n]/[\1_n^\top (\Int-\Pi)\1_n]$.
\end{proposition}

\begin{proposition}(Exact Integration) For integrands of the form $f_{\mu,\nu} = \alpha + \beta^\top \varphi$ with $\alpha \in \rset, \beta \in \rset^s$, the SHCV estimate is exact: $\mathrm{SHCV}_n^p(\mu,\nu) = \slice_p^p(\mu,\nu)$
\end{proposition}

\begin{corollary}(Exact Integration for Elliptic distributions)
\end{corollary}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Wasserstein and Sliced-Wasserstein for Gaussian.}

For $\mu=\mathcal{N}(m_1,\Sigma_1)$ and $\nu=\mathcal{N}(m_2,\Sigma_2)$, we have
\begin{align}
    \Wass_2^2(\mu,\nu) = \|m_1 - m_2\|_2^2 + \mathrm{Tr}[\Sigma_1 + \Sigma_2 - 2(\Sigma_1^{1/2}\Sigma_2\Sigma_1^{1/2})^{1/2}]
\end{align}
The $1$d projected distributions for $\theta \in \mathbb{S}^{d-1}$ are $\theta^\top \mu \sim \mathcal{N}(\theta^\top m_1, \theta^\top \Sigma_1 \theta)$ and $\theta^\top \nu \sim \mathcal{N}(\theta^\top m_2, \theta^\top \Sigma_2 \theta)$
\begin{align}
\Wass_2^2(\theta_{\#}^\star\mu,\theta_{\#}^\star\nu)= (\theta^\top(m_1-m_2))^2 + (\sqrt{\theta^\top \Sigma_1 \theta}- \sqrt{\theta^\top \Sigma_2 \theta})^2
\end{align}

On the one hand we have $(\theta^\top(m_1-m_2))^2 = (m_1-m_2)^\top \theta \theta^\top (m_1-m_2)$ and since $ \int_{\mathbb{S}^{d-1}} \theta \theta^\top \mathrm{d}\sigma(\theta) = \mathrm{I}_d/d$ we have
\begin{align*}
    \int_{\mathbb{S}^{d-1}} (\theta^\top(m_1-m_2))^2 \mathrm{d}\sigma(\theta) = \frac{1}{d} \|m_1 - m_2\|_2^2
\end{align*}
On the other hand we have
\begin{align*}
 (\sqrt{\theta^\top \Sigma_1 \theta}- \sqrt{\theta^\top \Sigma_2 \theta})^2 
 &= \theta^\top \Sigma_1 \theta + \theta^\top \Sigma_2 \theta - 2 [(\theta^\top \Sigma_1 \theta)(\theta^\top \Sigma_2 \theta)]^{1/2} \\
 &= q_{\Sigma_1}(\theta) + q_{\Sigma_2}(\theta) - 2 [q_{\Sigma_1}(\theta)q_{\Sigma_2}(\theta)]^{1/2}
\end{align*}
where $q_{\Sigma}(\theta)=\theta^\top \Sigma \theta$ is the quadratic form associated to $\Sigma$. After computations I found that 
\begin{align*}
    \expec_{\theta \sim \mathcal{U}(\mathcal{S}^{d-1})}[q_{\Sigma}(\theta)] = \int_{\mathbb{S}^{d-1}} (\theta^\top \Sigma \theta) \mathrm{d}\sigma(\theta) =\frac{\mathrm{Tr}(\Sigma)}{d}, \qquad \expec_{\theta \sim \mathcal{U}(\mathcal{S}^{d-1})}[q_{\Sigma}(\theta)^2] = \frac{\mathrm{Tr}(\Sigma)^2 + \mathrm{Tr}(\Sigma^2)}{d(d+1)}
\end{align*}

For a general covariance matrix $\Sigma$, we can diagonalize it as $\Sigma = P D P^\top$ with orthogonal $P \in O_d(\rset)$ so that $\theta^\top \Sigma \theta = \theta^\top (P D P^\top) \theta = (P^\top \theta)^\top D (P^\top \theta)$. Since $\theta \sim \mathcal{U}(\mathbb{S}^{d-1})$ and $P \in O_d(\rset)$ then $(P^\top \theta) \sim \mathcal{U}(\mathbb{S}^{d-1})$. To prove this, note that $X=Y/\|Y\|_2$ with $Y\sim \mathcal{N}(0,\mathrm{I}_d)$ so that $PY\sim \mathcal{N}(0,\mathrm{I}_d)$ and $\|PY\|_2 = \|Y\|_2$ which implies $PX = PY/\|PY\|_2 \sim \mathcal{U}(\mathbb{S}^{d-1})$

The problem is solved as soon as we find a closed form for the following problem: Given two symmetric positive semi-definite matrices $\mathbf{A}$ and $\mathbf{B}$, define the (Mahalanobis) norms as $\|\theta\|_\mathbf{A} = \sqrt{\theta^\top \mathbf{A} \theta}$ and $\|\theta\|_\mathbf{B} = \sqrt{\theta^\top \mathbf{B} \theta}$ we need to compute
\begin{align*}
    \expec_{\theta \sim \mathcal{U}(\mathcal{S}^{d-1})}[\|\theta\|_\mathbf{A}\|\theta\|_\mathbf{B}] 
    &= \expec[ \sqrt{\theta^\top \mathbf{A} \theta}  \sqrt{\theta^\top \mathbf{B} \theta}] \\
    &= \expec[ \sqrt{\theta^\top \mathbf{A} (\theta \theta^\top)\mathbf{B} \theta}]
\end{align*}

\#\#\#\#\#\#\# CONJECTURE (TRUE for diagonal covariances numerically) \#\#\#\#\#\#\#

 Sliced Wasserstein between general multivariate Gaussian  $\mathrm{SW}_2^2(\mu,\nu)$ is proportional with a factor $(1/d)$ to the Wasserstein (I am not 100\% sure of that)
\begin{align*}
    \mathrm{SW}_2^2(\mathcal{N}(m_1,\Sigma_1),\mathcal{N}(m_2,\Sigma_2) 
    &= \frac{1}{d} \Wass_2^2(\mathcal{N}(m_1,\Sigma_1),\mathcal{N}(m_2,\Sigma_2)
\end{align*}

\js{This is incorrect I believe. In general, I believe the left-hand side is bounded by the right-hand side and there is equality if and only if the two covariance matrices are proportional. Numerically, the difference may be small, however; try for instance $\Sigma_1 = \begin{bmatrix} 1 & 0 \\ 0 & 2 \end{bmatrix}$ and $\Sigma_2 = \begin{bmatrix} 2 & 0 \\ 0 & 1 \end{bmatrix}$. Is it worth typing out a proof?}


\iffalse
	\begin{theorem}[Non-asymptotic bound] \label{th:non_asymp_bound}
    \js{To be removed.}
		Let $p \in [1,\infty)$ and $\mu, \nu \in \mathcal{P}_p(\rset^d)$. Let $2 L$ be the maximum degree of spherical harmonics.  Then, for all $\delta \in (0,1)$ and all integer $n$ such that
		\begin{equation*}
			n \ge \max \cbr{18 |\sphere|^{-1} s  \log(4s/ \delta), 75 s \log(4/\delta)}
		\end{equation*}
		we have, with probability at least $1-\delta$,
		\begin{align*}
			%\MoveEqLeft[3]
   &\left|\SHCV_{n,L}^p({\mu,\nu}) - \SW_p^p(\mu,\nu)\right| \nonumber \le C_1 \sqrt{\log(8/\delta)} \frac{M_p(\mu,\nu) d}{L \sqrt{n}} \nonumber\\
			&+ \frac{C_2 s d M_p(\mu,\nu)}{L n} \sqrt{\frac{\log(8s/\delta) \log(4/\delta)}{|\sphere|}} ,
		\end{align*}
	where $s=\sum_{\ell = 2, 4, \ldots, 2L}  N_{\ell}^d= \binom{2L+d-1}{d-1}-1$ and constants $C_1, C_2$ are specified in the proof of the theorem.
	\end{theorem}
\fi
